Classification from Pairwise Similarities/Dissimilarities and Unlabeled Data via Empirical Risk Minimization

Pairwise similarities and dissimilarities between data points might be easier to obtain than fully labeled data in real-world classification problems, e.g., in privacy-aware situations. To handle such pairwise information, an empirical risk minimization approach has been proposed, giving an unbiased estimator of the classification risk that can be computed only from pairwise similarities and unlabeled data. However, this direction cannot handle pairwise dissimilarities so far. On the other hand, semi-supervised clustering is one of the methods which can use both similarities and dissimilarities. Nevertheless, they typically require strong geometrical assumptions on the data distribution such as the manifold assumption, which may deteriorate the performance. In this paper, we derive an unbiased risk estimator which can handle all of similarities/dissimilarities and unlabeled data. We theoretically establish estimation error bounds and experimentally demonstrate the practical usefulness of our empirical risk minimization method.

==> contents/sdu_gen.tex <==
\section{Proposed Method}
\label{sec:propose}
In this section, we propose SDU classification, 
where the classification risk is estimated from similar and dissimilar pairs and unlabeled data.
For the preparation to construct SDU classification,
we extend SU classification to DU and SD classification first.

\subsection{DU and SD classification}
\label{sec:dusd}
As well as SU classification, the classification risk can be estimated only from
dissimilar pairs and unlabeled data (DU),
or similar pairs and dissimilar pairs (SD) as follows.

\begin{theorem}
The classification risk in Eq.\,\eqref{eq:exp_pn_risk} can be equivalently represented as
\begin{equation}
\begin{split}
    R_{\DU}(f) = & \pi_\D \E_{(X,X') \sim p_\D(\boldsymbol{x}, \boldsymbol{x}')}
    \left[
            - \frac{\widetilde{\mathcal{L}}(f(X)) + \widetilde{\mathcal{L}}(f(X'))}{2}
    \right] \\
    & + \E_{X \sim p_\U(\boldsymbol{x})}
    \left[
            \mathcal{L}(f(X), +1)
    \right],
\end{split}
\end{equation}
\begin{equation}
\begin{split}
& R_{\rm SD}(f) \\
    & = \pi_\S \E_{(X,X') \sim p_\S(\boldsymbol{x}, \boldsymbol{x}')}
    \left[
            \frac{\mathcal{L}(f(X), +1) + \mathcal{L}(f(X'), +1)}{2}
    \right] \\
    & \quad + \pi_\D \E_{(X,X') \sim p_\D (\boldsymbol{x}, \boldsymbol{x}')}
    \left[
            \frac{\mathcal{L}(f(X), -1) + \mathcal{L}(f(X'), -1)}{2}
    \right],
\end{split}
\end{equation}
where $\mathcal{L}(z, t)$ and $\widetilde{\mathcal{L}} (z)$ are defined in Theorem~\ref{theo:su}.
\end{theorem}
We can train a classifier by minimizing the empirical version of $R_\DU$ or $R_\SD$, $\widehat{R}_\DU$ or $\widehat{R}_\SD$,
obtained from $(\mathfrak{D}_\D, \mathfrak{D}_\U)$ or $(\mathfrak{D}_\S, \mathfrak{D}_\D)$.
We call the training with these risks DU classification and SD classification, respectively.

\subsection{SDU classification}
We propose SDU classification by combining SU, DU, and SD classification.
The main idea of our method is to combine risks obtained from SU, DU and SD data in a similar manner to Positive-Negative-Unlabeled (PNU) classification~\cite{sakai2017semi}.

% With a positive real value $\gamma \in [0,1]$,
% we define the following three representations of the classification risk.
With positive real values  $ \boldsymbol{\gamma} = \{ \gamma_1,\gamma_2,\gamma_3 \} $ which satisfy the condition $\gamma_1 + \gamma_2 + \gamma_3 = 1$, 
we define the following representation of the classification risk.
\begin{equation}
\label{eq:risk_sdu}
    R_{\rm SDU}^{\boldsymbol{\gamma}} (\w) = \gamma_1 R_{\rm SU}(\w) + \gamma_2 R_{\rm DU}(\w) + \gamma_3 R_{\rm SD}(\w).
\end{equation}
We call the training with the empirical version of $R_{\rm SDU}$, $\widehat{R}_{\rm SDU}$, SDU classification.
% Here, one spontaneous question is how to choose $\boldsymbol{\gamma}$.
% From estimation error bounds analysis, 
% we can claim that the combination of SD and DU classification is the most promising,
% which is discussed in ec.\,\ref{sec:theo_sudusd}.
% We can claim the combination of SD and DU risks is the most promising from the point of view of estimation error bounds.
% discuss the details in Sec.\,\ref{sec:theo_sudusd}.

\begin{comment}
\begin{align}
\label{eq:risk_SDSU}
    & R_{\rm SDSU}^{\gamma}(f) \defeq (1-\gamma) R_{\rm SD}(f) + \gamma R_{\rm SU}(f), \\
\label{eq:risk_SDDU}
    & R_{\rm SDDU}^{\gamma}(f) \defeq (1-\gamma) R_{\rm SD}(f) + \gamma R_{\rm DU}(f), \\
\label{eq:risk_SUDU}
    & R_{\rm SUDU}^{\gamma}(f) \defeq (1-\gamma) R_{\rm SU}(f) + \gamma R_{\rm DU}(f).
\end{align}
We call the training with these risks SDSU classification, SDDU classification, and SUDU classifications, respectively.
Here, one spontaneous question is that which one is the most promising algorithm.
\end{comment}
% Here, one spontaneous question is that which one is the most promising algorithm.
%We call the training with these risks SDSU classification, SDDU classification, and SUDU classifications, respectively.
%Here, one spontaneous question is that which one is the most promising algorithm.
%We can claim the combination of SD and DU classification is the most promising from the point of view of estimation error bounds.
%We discuss the details in Sec.\,\ref{sec:theo_sudusd}.

\subsection{Practical Implementation}
We investigate the objective function when we use a linear classifier 
$f(\bx) = {\w}^{\top} \phi(\bx) + b$, 
where $\w \in \R^k$ and $b \in \R$ are parameters and $\phi: \R^d \rightarrow \R^k$ is a mapping function.
% For simplicity, we consider the following generalized optimization problem,
% With positive real values  $ \boldsymbol{\gamma} = \{ \gamma_1,\gamma_2,\gamma_3 \} $ which satisfy the condition $\gamma_1 + \gamma_2 + \gamma_3 = 1$, we denote our optimization problem by
% With the empirical risk $\widehat{R}_{\rm SDU}$, we denote our optimization problem by
Our optimization problem is denoted by
\begin{equation}
\label{eq:min_j}
\min_{\w} \hat{J}^{\boldsymbol{\gamma}}(\w),
\end{equation}
where
\begin{align}
 & \hat{J}^{\boldsymbol{\gamma}}(\w) = \hat{R}_{\rm SDU}^{\boldsymbol{\gamma}}(\w) + \frac{\lambda}{2} \| \w \|^2.
\label{eq:obj}
% & \hat{R}_{\rm SDU}^{\boldsymbol{\gamma}} (\w)
% = \gamma_1 \hat{R}_{\rm SU}(\w) + \gamma_2 \hat{R}_{\rm DU}(\w) + \gamma_3 \hat{R}_{\rm SD}(\w).
\end{align}
Here, $\lambda > 0$ is a parameter of L2 regularization.
%When $\gamma_1 = 0$, $\gamma_2=0$ and $\gamma_3=0$, 
%this optimization corresponds to SDDU, SDSU, SUDU classification, respectively.

From now on, we assume the loss function is margin loss function.
As defined in \cite{mohri2018foundations}, we call $\ell$ is a margin loss function if there exists $\psi: \R \rightarrow \R_+$ such that $\ell(z,t)=\psi(tz).$
In general, the optimization problem in Eq.\,\eqref{eq:min_j} is not a convex problem.
However, if we choose $\ell$ satisfies a certain property, the optimization problem gets convex. 
\begin{theorem}
Suppose that the loss function is second order differentiable and satisfies following condition.
\begin{equation}
\label{eq:loss_assumption}
    \ell(z, +1) - \ell(z, -1) = -z.
\end{equation}
Then, the optimization problem in Eq.\,(\ref{eq:min_j}) is a convex problem.
\end{theorem}
Next, we consider the case of squared loss and double hinge loss, which satisfy the condition in Eq.\,\eqref{eq:loss_assumption}.

\subsubsection{Squared Loss}
Suppose that we use squared loss defined by
\begin{equation}
    \label{eq:loss_sq}
    \ell_{\rm SQ}(z, t) = \frac{1}{4}(tz-1)^2.
\end{equation}
Then, the objective function in $\widehat{J}^{\boldsymbol{\gamma}}(\w)$ can be written as
\begin{equation}
    \begin{split}
    \widehat{J}^{\boldsymbol{\gamma}}(\w)
    & = \frac{1}{4} \w^\top \left\{\gamma_3 \left( \frac{\pi_\S}{2n_\S}X_\S^\top X_\S + \frac{\pi_\D}{2n_\D}X_\D^\top X_\D \right) \right. \\
  &  \left. + \frac{\gamma_1 + \gamma_2}{n_\U} X_\U^\top X_\U + 2 \lambda I \right\} \w \\
  & +\frac{1}{\pi_+ - \pi_-}\left\{ -\frac{\pi_\S}{2 n_\S}\left( \gamma_1 + \frac{\gamma_3}{2} \right)  X_\S^\top \mathbf{1} \right.\\
  & \left. + \frac{\pi_\D}{2 n_\D}\left( \gamma_2 + \frac{\gamma_3}{2} \right) X_\D^\top \mathbf{1}
  + \frac{1}{2 n_\U}\left( \gamma_1 - \gamma_2 \right) X_\U^\top \mathbf{1} 
  \right\} \w \\
  & +\text{const},
\end{split}
\end{equation}
\begin{comment}
\begin{equation}
\begin{split}
    & \resizebox{1.1 \linewidth}{!}{$\frac{1}{4} \w^\top \left\{\frac{\gamma_3}{2} \left( \frac{\pi_\S}{n_\S}X_\S^\top X_\S + \frac{\pi_\D}{n_\D}X_\D^\top X_\D \right) 
     + \frac{\gamma_1 + \gamma_2}{n_\U} X_\U^\top X_\U + 2 \lambda I \right\} \w $}\\
   & \resizebox{1. \linewidth}{!}{$+\frac{1}{\pi_+ - \pi_-} \left\{ -\frac{\pi_\S}{2 n_\S}\left( \gamma_1 + \frac{\gamma_3}{2} \right)  X_\S^\top \mathbf{1} + \frac{\pi_\D}{2 n_\D}\left( \gamma_2 + \frac{\gamma_3}{2} \right) X_\D^\top \mathbf{1} \right.$} \\ 
   & \resizebox{0.5 \linewidth}{!}{$\left. + \frac{1}{2 n_\U}\left( \gamma_1 - \gamma_2 \right) X_\U^\top \mathbf{1} \right\} \w + \text{const}$},
\end{split}
\end{equation}
\begin{equation}

\end{equation}
\end{comment}
where 
$X_\S \defeq [\phi(\bx_{\S,1}),\phi(\bx'_{\S,1}),\dots, \phi(\bx_{\S,n_\S}),\phi(\bx'_{\S,n_\S})]^\top$, 
$X_\D \defeq [\phi(\bx_{\D,1}),\phi(\bx'_{\D,1}),\dots, \phi(\bx_{\D,n_\D}),\phi(\bx'_{\D,n_\D})]^\top$,
$X_\U \defeq [\phi(\bx_{\U,1}),\dots, \phi(\bx_{\U, n_\U})]^\top$, 
$\mathbf{1}$ is the vector whose elements are all ones,
and $I$ is the indentity matrix. 
As this function has quadratic form with respect to $\w$,
the solution of this minimization problem can be obtained analytically.

\begin{comment}
    \begin{equation}
    \begin{split}
    \hat{\w} = & \frac{1}{\pi_+ - \pi_-} 
     \left\{\gamma_3 \left( \frac{\pi_\S}{2n_\S}X_\S^\top X_\S + \frac{\pi_\D}{2n_\D}X_\D^\top X_\D \right) \right. \\
      & \left. + \frac{\gamma_1 + \gamma_2}{n_\U} X_\U^\top X_\U + 2 \lambda I \right\}^{-1} \\
    &\left\{ \frac{\pi_\S}{n_\S}\left( \gamma_1 + \frac{\gamma_3}{2} \right)  X_\S^\top \mathbf{1} + \frac{\pi_\D}{n_\D}\left( \gamma_2 + \frac{\gamma_3}{2} \right) X_\D^\top \mathbf{1} \right. \\
    & \left.  + \frac{1}{n_\U}\left( \gamma_1 - \gamma_2 \right) X_\U^\top \mathbf{1}
      \right\}.
    \end{split}
    \end{equation}
\end{comment}


\subsubsection{Double Hinge Loss}
Standard hinge loss $\ell_{\rm H}(z,t) = \max(0, -tz)$ does not satisfy condition in Eq.\,\eqref{eq:loss_assumption}. Instead, double hinge loss 
$\ell_{\rm DH}(z, t) = \max (-tz, \max (0, \frac{1}{2}-\frac{1}{2}tz)$
is proposed by \cite{du2015convex}.
When we use $\ell_{\rm DH}$,
we can solve the optimization problem in Eq.\,\eqref{eq:min_j}
by quadratic programming.
The detail is described in the supplementary material.
\begin{comment}
we can rewrite optimization problem in Eq.\,\eqref{eq:min_j} with slack variables
$\boldsymbol{\xi}=\{\boldsymbol{\xi}_\S,\boldsymbol{\xi}_\D,\boldsymbol{\xi}_\U \}$ and
$\boldsymbol{\eta}=\{\boldsymbol{\eta}_\S,\boldsymbol{\eta}_\D,\boldsymbol{\eta}_\U \}$
as follows:
\begin{equation}
\begin{split}
    \min_{\w, \boldsymbol{\xi}, \boldsymbol{\eta}} 
    & -\frac{\gamma_1 \pi_\S}{2 n_\S (\pi_+ - \pi_-)} \mathbf{1}^\top X_\S \w
    +\frac{\gamma_2 \pi_\D}{2 n_\D (\pi_+ - \pi_-)} \mathbf{1}^\top X_\D \w \\
    & + \frac{\gamma_3 \pi_+ \pi_\S}{2 n_\S (\pi_+ - \pi_-)} \mathbf{1}^\top \boldsymbol{\xi}_\S
      - \frac{\gamma_3 \pi_- \pi_\S}{2 n_\S (\pi_+ - \pi_-)} \mathbf{1}^\top \boldsymbol{\eta}_\S \\
    & - \frac{\gamma_3 \pi_- \pi_\D}{2 n_\D (\pi_+ - \pi_-)} \mathbf{1}^\top \boldsymbol{\xi}_\D
      + \frac{\gamma_3 \pi_+ \pi_\D}{2 n_\D (\pi_+ - \pi_-)} \mathbf{1}^\top \boldsymbol{\eta}_\D \\
    & + \frac{- \gamma_1 \pi_- + \gamma_2 \pi_+}{n_\U (\pi_+ - \pi_-)} \mathbf{1}^\top \boldsymbol{\xi}_\U
      + \frac{\gamma_1 \pi_+ - \gamma_2 \pi_-}{n_\U (\pi_+ - \pi_-)} \mathbf{1}^\top \boldsymbol{\eta}_\U \\
    & + \frac{1}{2}\|\w\|^2,
\end{split}
\end{equation}
\begin{equation}
\begin{split}
    \text{s.t.}~~~
    & \boldsymbol{\xi}_\S \geq 0,~\boldsymbol{\xi}_\S \geq \frac{1}{2} - \frac{1}{2}X_\S \w,~\boldsymbol{\xi}_\S \geq - X_\S \w, \\
    & \boldsymbol{\eta}_\S \geq 0,~\boldsymbol{\eta}_\S \geq \frac{1}{2} + \frac{1}{2}X_\S \w,~\boldsymbol{\eta}_\S \geq X_\S \w, \\
    & \boldsymbol{\xi}_\D \geq 0,~\boldsymbol{\xi}_\D \geq \frac{1}{2} - \frac{1}{2}X_\D \w,~\boldsymbol{\xi}_\D \geq - X_\D \w, \\
    & \boldsymbol{\eta}_\D \geq 0,~\boldsymbol{\eta}_\D \geq \frac{1}{2} + \frac{1}{2}X_\D \w,~\boldsymbol{\eta}_\D \geq X_\D \w, \\
    & \boldsymbol{\xi}_\U \geq 0,~\boldsymbol{\xi}_\U \geq \frac{1}{2} - \frac{1}{2}X_\U \w,~\boldsymbol{\xi}_\U \geq - X_\U \w, \\
    & \boldsymbol{\eta}_\U \geq 0,~\boldsymbol{\eta}_\U \geq \frac{1}{2} + \frac{1}{2}X_\U \w,~\boldsymbol{\eta}_\U \geq X_\U \w,
\end{split}
\end{equation}
where $\geq$ for vectors indicates element-wise inequality.
Note that this optimization problem is a quadratic problem.
\end{comment}


\subsection{Class Prior Estimation}
Though we have to know the class prior $\pi_+$ before training
for calculation of empirical risks $R_\SD$, $R_\SU$, and $R_\DU$,
$\pi_+$ can be estimated from the number of similar $n_\S$ and dissimilar data $n_\D$.
First, $\pi_+$ and $\pi_\S$ has following relationship.
\begin{equation}
\label{eq:cpe}
    \pi_+ = 
    \begin{cases}
    \frac{1 + \sqrt{1 - 2(1-\pi_\S)}}{2} & (\pi_+ \geq 0.5) \\
    \frac{1 - \sqrt{1 - 2(1-\pi_\S)}}{2} & (\pi_+ < 0.5)
    \end{cases},
\end{equation}
The above relationship is yielded from 
$2\pi_\S - 1 = \pi_\S - \pi_\D = (\pi_+ - \pi_-) = (2\pi_+ - 1)^2$.
Note that $\widehat{\pi}_\S = {n_\S} / ({n_\S + n_\D})$ is an unbiased estimator of $\pi_\S$.
Thus, $\pi_+$ ca be estimated by plugging $\widehat{\pi}_\S$ into Eq.\,\eqref{eq:cpe}.
%From $\widehat{\pi}_\S = {n_\S} / ({n_\S + n_\D})$ estimated 
%from the number of similar and dissimilar pairs, 
%i.e., $n_\S$ and $n_\D$,
%we obtain estimated $\widehat{\pi}_+$.
% Even if we don't know true class prior in practice 
% and choose opposite value for ,
% trained classifier output predict completely flipped class label.
% While we don't always know whether $\pi_+ \geq 1/2$ in practice,
% we can classify unseen data into two classes.
% Even in such cases, we can classify unseen data into two classes, 
% but we cannot know the mapping between true positive and negative class, and our predicted positive and negative class.
% That will satisfy our demand for most cases.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
